Self-consistent modeling of runaway electron generation in massive gas injection scenarios in ASDEX Upgrade

We present the first successful simulation of a induced disruption in ASDEX Upgrade from massive material injection (MMI) up to established runaway electron (RE) beam, thus covering pre-thermal quench, thermal quench and current quench (CQ) of the discharge. For future high-current fusion devices such as ITER, the successful suppression of REs through MMI is of critical importance to ensure the structural integrity of the vessel. To computationally study the interplay between MMI, background plasma response, and RE generation, a toolkit based on the 1.5D transport code coupling ASTRA-STRAHL is developed. Electron runaway is described by state-of-the-art reduced kinetic models in the presence of partially ionized impurities. Applied to argon MMI in ASDEX Upgrade discharge #33108, key plasma parameters measured experimentally, such as temporal evolution of the line averaged electron density, plasma current decay rate and post-CQ RE current, are well reproduced by the simulation presented. Impurity ions are transported into the central plasma by the combined effect of neoclassical processes and additional effects prescribed inside the $q = 2$ rational surface to explain experimental time scales. Thus, a thermal collapse is induced through strong impurity radiation, giving rise to a substantial RE population as observed experimentally.

==> 04_bolo_s13.tex <==
\begin{figure}
	\centering
	\includegraphics[scale=1]{04_bolo_s13_fig.pdf}
	\centering
	\caption[Radiation measurements by AXUV diodes in sector 13]{%
		\label{fig:bolo_s13}
		Radiation measurements of the individual channels of the AXUV photodiodes in sector 13 (see fig.~\ref{fig:diag_geom} for their line-of-sights). Channels 1 to 14 capture LFS radiation, i.e. their lines-of-sight intersect the equatorial plane beyond the magnetic axis, whereas channels 15 to 32 cover the HFS. Core radiation is captured by channels 6 to 30. Note, that this classification is valid only in the very early phase of the disruption. The Ar injected reaches the LFS-LCFS at $t = 1~{\rm ms}$ (a), ionizes and re-distributes poloidally (b), eventually causing a thermal collapse at $t = 3~{\rm ms}$ (c), followed by strong central radiation (d).}
\end{figure}
